Taylorized Training: Towards Better Approximation of Neural Network Training at Finite Width

We propose \emph{Taylorized training} as an initiative towards better understanding neural network training at finite width. Taylorized training involves training the $k$-th order Taylor expansion of the neural network at initialization, and is a principled extension of linearized training---a recently proposed theory for understanding the success of deep learning. We experiment with Taylorized training on modern neural network architectures, and show that Taylorized training (1) agrees with full neural network training increasingly better as we increase $k$, and (2) can significantly close the performance gap between linearized and full training. Compared with linearized training, higher-order training works in more realistic settings such as standard parameterization and large (initial) learning rate. We complement our experiments with theoretical results showing that the approximation error of $k$-th order Taylorized models decay exponentially over $k$ in wide neural networks.

==> Sections/experiments.tex <==
\section{Experiments}
\label{section:experiments}

\begin{table*}
  \small
  \centering
  \begin{tabular}{l@{\ \ }|@{\ \ }c@{\ \ }c@{\ \ }| c@{\ \ }c@{\ \ }c@{\ \ }c@{\ \ }c@{\ \ }c@{\ \ } c@{\ \ } @{\ \ }c@{\ \ }c@{\ \ }}
    \toprule
    Name & Architecture & Params& Train For & Batch & Accuracy & Opt &
                                                                       Rate
    & Grad Clip & LR Decay Schedule \\ 
    \midrule
    CNNTHIN & CNN-4-128 & 447K & 200 epochs & 256 & 81.6\%
                                                          & SGD & 0.1
    & 5.0
                                                                       
    & 10x drop at 100, 150 epochs \\
   CNNTHICK & CNN-4-512 & 7.10M & 160 epochs & 64 & 85.9\%
                                                          & SGD &  0.1
    & 5.0
    & 10x drop
    at 80, 120 epochs\\
    \midrule
    WRNTHIN & WideResNet-16-4-128 & 3.22M & 200 epochs & 256 & 88.1\% &
                                                                  SGD
                                                                     &
                                                                       1e-1.5
    & 10.0 & 10x drop at 100, 150 epochs \\ 
    WRNTHICK & WideResNet-16-8-256 & 12.84M & 160 epochs & 64 & 91.7\%
                                                               & SGD & 
                                                                    1e-1.5
    & 10.0 & 10x drop at 80, 120 epochs \\ 
    \bottomrule
  \end{tabular}
  \caption{{\bf Our architectures and training setups.} CNN-$L$-$C$ stands for a
  CNN with depth $L$ and $C$ channels per
  layer. WideResNet-$L$-$k$-$C$ stands for a WideResNet with depth $L$, widening
  factor $k$, and $C$ channels in the first convolutional
  layer.}
  \label{table:architectures}
\end{table*}

We experiment with Taylorized training on convolutional and residual
networks for the image classification task on CIFAR-10. % Our
% experiments demonstrate the advantage of Taylorized training in terms
% of both approximating full training and reaching good test performance
% in practical training regimes.

\subsection{Basic setup}
We choose four representative architectures for the image
classification task: two CNNs with 4 layers + Global Average Pooling
(GAP) with width $\set{128, 512}$, and two
WideResNets~\cite{zagoruyko2016wide} with depth 16 and different
widths as well. All networks use standard parameterization and are
trained with the cross-entropy loss\footnote{Different from prior work
  on linearized training which primarily focused on the squared
  loss~\cite{arora2019exact,lee2019wide}.}. We optimize the training
loss using SGD with a large initial learning rate + learning rate
decay.\footnote{We also use gradient clipping with a large clipping
  norm in order to prevent occasional gradient blow-ups.}

% \yub{Highlight we use practical training regimes? (large lr and
%   standard parameterization.)}
For each architecture, the
initial learning rate was tuned within
$\set{10^{-2}, 10^{-1.5}, 10^{-1}, 10^{-0.5}}$ and chosen to be the
largest learning rate under which the full neural network can stably
train (i.e. has a smoothly decreasing training loss). We use standard
data augmentation (random crop, flip, and standardize) as a
optimization-independent way for
improving generalization.
% \footnote{As opposed
%   to weight decay which can potentially twist the training trajectory
% differently for full and Taylorized training.}
Detailed training
settings for each architecture are summarized in
Table~\ref{table:architectures}.

% \paragraph{Training Taylorized models from a common initialization}
\paragraph{Methodology}
For each architecture, we train Taylorized models of order
$k\in\set{1,2,3,4}$ (referred to as \{linearized, quadratic, cubic,
quartic\} models) from the {\bf same initialization} as full training
using the {\bf exact same optimization setting} (including learning
rate decay, gradient clipping, minibatching, and data augmentation
noise). This allows us to eliminate the effects of optimization setup
and randomness, and examine the agreement between Taylorized and full
training in identical settings.

\subsection{Approximation power of Taylorized training}
\label{section:approximation-exp}
% \yub{better subtitle?}
We examine the approximation power of Taylorized training through
comparing Taylorized training of different orders in terms of both the
training trajectory and the test performance.

\paragraph{Metrics}
We monitor the training loss and test accuracy for
both full and Taylorized training. We also evaluate the approximation
error between Taylorized and
full training quantitatively through the following similarity metrics
between models:  % in both the parameter space and the function space:
\begin{itemize}
\item Cosine similarity in the parameter space, defined as
  \begin{equation*}
    \cosparam_t \defeq \frac{\<\theta^{(k)}_t - \theta_0,
      \theta_t - \theta_0\>}{\big\|\theta^{(k)}_t -
        \theta_0\big\|\big\|\theta_t - \theta_0\big\|},
  \end{equation*}
  where (recall~\eqref{equation:taylorized-training}
  and~\eqref{equation:full-training}) $\theta^{(k)}_t$ and
  $\theta_t$ denote the parameters in $k$-th order 
  Taylorized training and full training, and $\theta_0$ is their
  common initialization.
\item Cosine similarity in the function space, defined as
  \begin{equation*}
    \cosfunc_t \defeq \frac{\<f^{(k)}_{\theta^{(k)}_t} - f_{\theta_0},
      f_{\theta_t} -
      f_{\theta_0}\>}{\big\|f^{(k)}_{\theta^{(k)}_t}-
        f_{\theta_0}\big\|\big\|f_{\theta_t} - 
        f_{\theta_0}\big\|},
  \end{equation*}
  where we have overloaded the notation
  $f\in\R^{C\times n_{\rm test}}$ (and similarly $f^{(k)}$) to denote
  the output (logits) of a model on the test dataset\footnote{We
    centralized (demeaned) the logits for each example along the
    classification axis so as to remove the effect of the invariance
    in the softmax mapping.
  }.
\end{itemize}
% For the purpose of comparing models, these two metrics are
% complementary to each other: the function space similarity measures
% distance between models in a sensible way (by comparing test
% predictions), though it can be strongly tied to the performance of the
% model (two high-performing models would output similar logits); the
% parameter space similarity looks at the raw parameter space without
% knowledge about the actual architecture, yet is itself a metric that
% is more independent of the performance of the model.

\begin{figure*}
  \centering
    \includegraphics[width=0.24\textwidth]{plots/cnn_thin/trainloss.pdf}
    \includegraphics[width=0.24\textwidth]{plots/cnn_thin/testacc.pdf}
    \includegraphics[width=0.24\textwidth]{plots/cnn_thin/cosparam.pdf}
    \includegraphics[width=0.24\textwidth]{plots/cnn_thin/cospred.pdf}
    \caption{{\bf $k$-th order Taylorized training approximates full
      training increasingly better with $k$ on the CNNTHIN
      model.} Training statistics are plotted for \{\textbf{{\color{C0}
          full}, {\color{C1} linearized}, {\color{C2} quadratic},
        {\color{C3} cubic}, {\color{C4} quartic}}\} models. Left to
      right: (1) training loss; (2) test accuracy; (3) cosine
      similarity between Taylorized and full training in the parameter
      space; (4) cosine similarity between Taylorized and full
      training in the function (logit) space. All models are trained on
      CIFAR-10 for 39200 steps, and a 10x learning rate decay happened
      at step \{19600, 29400\}.}
  \label{figure:cnnthin-approximation}
\end{figure*}


\begin{table*}
  \centering
  \begin{tabular}{c|c|c|c|c}
    \hline
    Architecture & CNNTHIN & CNNTHICK & WRNTHIN & WRNTHICK \\ 
    \hline
    Linearized ($k=1$) & 41.3\% & 49.0\% & 50.2\% & 55.3\% \\
    Quadratic ($k=2$) & 61.6\% & 70.1\% & 65.8\% & 71.7\% \\
    Cubic ($k=3$) & 69.3\% & 75.3\% & 72.6\% & 76.9\% \\
    Quartic ($k=4$) & 71.8\% & 76.2\% & 75.6\% & 78.7\% \\
    \hline
    Full network & 81.6\% & 85.9\% & 88.1\% & 91.7\% \\
    \hline
  \end{tabular}
  \caption{{\bf Final test accuracy on CIFAR-10 for Taylorized models
    trained under the same optimization setup as full neural
    nets.} Details about the architectures and their training setups
    can be found in Table~\ref{table:architectures}.}
  \label{table:taylorized-performance}
\end{table*}

\vspace{-0.3cm}
\paragraph{Results}
Figure~\ref{figure:cnnthin-approximation} plots training and
approximation metrics for full and Taylorized training on the CNNTHIN
model in

% It can be seen that
% Taylorized models are good interpolators of linearized and full
% training --
Observe that Taylorized models are much better approximators than
linearized models in both the parameter space and the function
space---both cosine similarity curves shift up as we increase $k$ from
1 to 4. Further, for the cubic and quartic 
models, the cosine similarity in the logit space stays above 0.8 over
the entire training trajectory (which includes both weakly and
strongly trained models), suggesting a fine agreement between
higher-order Taylorized training and full training. Results
for \{CNNTHICK, WRNTHIN, WRNTHICK\} are qualitatively similar and are
provided in Appendix~\ref{appendix:approximation}.


We further report the final test performance of the Taylorized models
on all architectures in Table~\ref{table:taylorized-performance}. We
observe that
% \vspace{-0.1cm}
\begin{enumerate}[(1)]
\item Taylorized models can indeed close the performance gap between
  linearized and full training: linearized models are typically
  30\%-40\% worse than fully trained networks, whereas quartic (4th
  order Taylorized) models are within \{10\%, 13\%\} of a fully trained
  network on \{CNNs, WideResNets\}.
\item All Taylorized models can benifit from increasing the width
  (from CNNTHIN to CNNTHICK, and WRNTHIN to WRNTHICK), but the
  performance of higher-order models ($k=3,4$) are generally less
  sensitive to width than lower-order models ($k=1,2$), suggesting
  their realisticness for explaining the training behavior of
  practically sized finite-width networks.
\end{enumerate}

\paragraph{On finite- vs. infinite-width linearized models}
We emphasize that the performance of our baseline linearized models in
Table~\ref{table:taylorized-performance}  (40\%-55\%) is at finite
width, and is thus not directly comparable to
existing results on infinite-width linearized models such as
CNTK~\cite{arora2019exact}. %  or its enhanced
% versions~\cite{li2019enhanced}
It is possible to achieve stronger results with finite-width
linearized networks by using the NTK parameterization, which more
closely resembles the infinite width limit. However, full neural net
training with this re-parameterization results in significantly
weakened performance, suggesting its unrealisticness. The
best documented test accuracy of a finite-width linearized network on
CIFAR-10 is $\sim$65\%~\cite{lee2019wide}, and due to the NTK
parameterization, the neural network trained under these same settings
only reached $\sim$70\%. In contrast, our best higher order models can
approach 80\%, and are trained under realistic settings where a neural
network can reach over 90\%. 

%Indeed, it has been observed that finite-width linearized networks are hard to optimize (e.g. to nearly 0 training loss) because of poorconditioning~\cite{chizat2019lazy}. 

\subsection{Agreement on layer movements}
% \yub{better subtitle?}

Layer importance, i.e. the contribution and importance of each layer
in a well-trained (deep) network, has been identified as a useful
concept towards building an architecture-dependent understanding on
neural network training~\cite{zhang2019all}. 
Here we demonstrate that
higher-order Taylorized training has the potential to lead to better
understandings on the layer importance in full training.

\paragraph{Method and result} We examine \emph{layer movements},
i.e. the distances each layer has travelled along training, and
illustrate it on both full and Taylorized
training.\footnote{Taylorized models $f^{(k)}_\theta$ are polynomials
  of $\theta$ where $\theta$ has the same shape as the base
  network. By a ``layer'' in a Taylorized model, we mean the partition
  that's same as how we partition $\theta$ into layers in the base
  network.}
In Figure~\ref{figure:layer-movement}, we plot the layer movements on
the CNNTHIN and WRNTHIN models. Compared with linearized training,
quartic training agrees with full training much better in the shape of
the layer movement curve, both at an early stage and at
convergence. Furthermore, comparing the layer movement curves between the
10th epoch and at convergence, quartic training seems to be able to
adjust the shape of the movement curve much better than linearized
training. % , suggesting their advantage for understanding layer
% importance.

% \paragraph{More on layer importance}
Intriguing results about layer importance has also been (implicitly)
shown in the study of infinite-width linearized models (i.e. NTK type
kernel methods). For example, it has been observed that the CNN-GP
kernel (which corresponds to training the top layer only) has
consistently better generalization performance than the CNTK kernel
(which corresponds to training all the
layer)~\cite{li2019enhanced}. In other words, when training an
extremely wide convolutional net on a finite dataset, training the
last layer only gives a better generalization performance (i.e. a
better implicit bias); existing theoretical work on linearized
training fall short of understanding layer importance in these
settings. We believe Taylorized training can serve as an (at
least empirically) useful tool towards understanding layer importance.


\begin{figure*}[t]
  \centering
  \begin{subfigure}[t]{0.48\textwidth}
    \centering
    \includegraphics[width=\textwidth]{plots/cnn_thin/layer_movement_step_2000.pdf}
    \caption{CNNTHIN at 10 epochs}
  \end{subfigure}
  \begin{subfigure}[t]{0.48\textwidth}
    \centering
    \includegraphics[width=\textwidth]{plots/wrn_small/layer_movement_step_2000.pdf}
    \caption{WRNSMALL at 10 epochs}
  \end{subfigure}
  \begin{subfigure}[t]{0.48\textwidth}
    \centering
    \includegraphics[width=\textwidth]{plots/cnn_thin/layer_movement_step_39200.pdf}
    \caption{CNNTHIN at convergence}
  \end{subfigure}
  \begin{subfigure}[t]{0.48\textwidth}
    \centering
    \includegraphics[width=\textwidth]{plots/wrn_small/layer_movement_step_39200.pdf}
    \caption{WRNSMALL at convergence}
  \end{subfigure}
  \caption{{\bf Layer movement of {\bf \color{C0} full NN},
    {\bf \color{C1} linearized}, and {\bf \color{C4} quartic}
    models.} Compared with linearized training, quartic (4th order)
    Taylorized training agrees with the full neural network much
    better in terms of layer movement, both at the initial stage and
    at convergence.}
  \label{figure:layer-movement}
\end{figure*}

==> Sections/intro.tex <==
\section{Introduction}
\label{section:intro}
Deep learning has made immense progress in solving artificial
intelligence challenges such as computer vision, natural language
processing, reinforcement learning, and so
on~\cite{lecun2015deep}. Despite this great success, fundamental
theoretical questions such as why deep networks train and
generalize well are only partially understood. 

A recent surge of research establishes the connection between
% the training trajectory of 
wide neural networks and their linearized
models. It is shown that wide neural networks can be trained in
a setting in which each individual weight only moves very slightly
(relative to itself), so that the evolution of the network can be
closely approximated by the evolution of the linearized model, which
when the width goes to infinity has a certain statistical limit
governed by its Neural Tangent Kernel (NTK).
Such a connection has led to provable optimization and generalization
results for wide neural nets
~\cite{li2018learning,jacot2018neural,du2018gradient,du2019gradient,zou2019gradient,lee2019wide,arora2019fine,allen2019learning},
and has inspired the design of new algorithms such as neural-based
kernel machines that achieve competitive results on benchmark learning
tasks~\cite{arora2019exact,li2019enhanced}.

% While the theory of linearized training is powerful, it is
While linearized training is powerful in theory, it is questionable
whether it really explains neural network training in practical
settings. Indeed, (1) the linearization theory requires small learning
rates or specific network parameterizations (such as the NTK
parameterization), yet in practice a large (initial) learning rate is
typically required in order to reach a good performance; (2) the
linearization theory requires a high width in order for the linearized
model to fit the training dataset and generalize, yet it is unclear
whether the finite-width linearization of practically sized network
have such capacities. Such a gap between linearized and full neural
network training has been identified in recent
work~\cite{chizat2019lazy,ghorbani2019linearized,
  ghorbani2019limitations,li2019towards}, and suggests the need for a
better model towards understanding neural network training in
practical regimes.

% Several concrete questions can be asked towards closing this gap:
% (1) does linearized training approximate full neural net training
% under the standard parameterization? (2) can we ``upgrade'' linearized
% training to a set of approxiamte dynamics that approximates standard
% neural net trainng better, yet still amenable to theoretical analysis?
% (3) is there a regime in which the approximation power of linearized
% trainig and our proposed training dynamics exhibit a significant gap?

Towards closing this gap, in this paper we propose and study
\emph{Taylorized training}, a principled generalization of linearized
training. For any neural network $f_\theta(x)$ and a given
initialization $\theta_0$, assuming sufficient smoothness, we can
expand $f_\theta$ around $\theta_0$ to the $k$-th order for any $k\ge
1$: 
\begin{align*}
  f_\theta(x) = \underbrace{f_{\theta_0}(x) + \sum_{j=1}^k
  \frac{\grad^j_\theta 
  f_{\theta_0}(x)}{j!}[\theta - \theta_0]^{\otimes j}}_{\defeq
  f^{(k)}_{\theta;\theta_0}(x)} + o\paren{\norm{\theta - \theta_0}^k}.
  \\ 
\end{align*}
The model $f^{(k)}_{\theta;\theta_0}(x)$ is exactly the linearized
model when $k=1$, and becomes $k$-th order polynomials of
$\theta-\theta_0$ that are increasingly better local approximations of
$f_\theta$ as we increase $k$. Taylorized training refers to training
these Taylorized models $f^{(k)}$ explicitly (and not necessarily
locally), and using it as a tool towards understanding the training of
the full neural network $f_\theta$. The hope with Taylorized training
is to ``trade expansion order with width'', that is, to hopefully
understand finite-width dynamics better by using a higher expansion
order $k$ rather than by increasing the width.
% \yub{How to properly cite here?}

In this paper, we take an empirical approach towards studying
Taylorized training, demonstrating its usefulness in understanding
finite-width full training\footnote{By full training, we mean the usual
  (non-Taylorized) training of the neural networks.}.
Our main contributions can be summarized
as follows:
\begin{itemize}
\item We experiment with Taylorized training on vanilla convolutional
  and residual networks in their practical training regimes (standard
  parameterization + large initial learning rate) on CIFAR-10. We show
  that Taylorized training gives increasingly better approximations of
  the training trajectory of the full neural net as we increase the
  expansion order $k$, in both the parameter space and the function
  space (Section~\ref{section:experiments}). This is not necessarily
  expected, as higher-order Taylorized models are no longer guaranteed
  to give better approximations when parameters travel significantly,
  yet empiricially they do approximate full training better.
\item We find that Taylorized models can significantly close the 
  performance gap between fully trained neural nets and their
  linearized models at finite width. Finite-width linearized networks
  typically has over 40\% worse test accuracy than their fully
  trained counterparts, whereas quartic (4th order) training is only
  10\%-15\% worse than full training under the same setup.
  % Our quadratic models achieve better
  % accuracy than the best known finite-width linearized models, and our
  % quartic (4th order) WideResNet can nearly match a fully trained
  % 4-layer CNN.
\item We demonstrate the potential of Taylorized training as a tool
  for understanding \emph{layer importance}. Specifically,
  higher-order Taylorized training agrees well with full training in
  layer movements, i.e. how far each layer travels from its
  initialization, whereas linearized training does not agree well. %  and
  % has a less adaptive layer movement curve throughout training.
\item We provide a theoretical analysis on the approximation power of
  Taylorized training (Section~\ref{section:theory}). We prove that
  $k$-th order Taylorized training 
  approximates the full training trajectory with error bound
  $O(m^{-k/2})$ on a wide two-layer network with width $m$. This
  extends existing results on linearized training and provides a
  preliminary justification of our experimental findings.
  % \item We propose specific parameterizations under which the
%   quadratic model approximates much better than the linearized
%   model. More generally, there exists specific parameterizations
%   under which the $k$-th order Taylorized model approximates the NN
%   training trajectory much better than all $\le k-1$-th order models.
\end{itemize}
\paragraph{Additional paper organization}
We provide preliminaries in Section~\ref{section:prelim}, review
linearized training in Section~\ref{section:linearized}, and describe
Taylorized training in more details in
Section~\ref{section:taylorized}. Additional experimental results are
reported in Appendix~\ref{appendix:additional-exps}.

% \yub{Add pointer to additional experiments in the appendix.}
\paragraph{A visualization of Taylorized training}
A high-level illustration of our results is provided in
Figure~\ref{figure:cnnthick-trajectory}, which visualizes the training
trajectories of a 4-layer convolutional neural network and its
Taylorized models. Observe that the linearized model struggles to
progress past the initial phase of training and is a rather poor
approximation of full training in this setting, whereas higher-order
Taylorized models approximate full training significantly better.


\begin{figure}
  \centering
  \includegraphics[width=\columnwidth]{plots/CNNTHICK_step_16000.pdf}
  \caption{{\bf Function space dynamics of a 4-layer CNN under
    full training ({\bf \color{C0} NN}) and Taylorized training of
    order 1-4 ({\bf \color{C1} linearized}, {\bf \color{C2}
      quadratic}, {\bf \color{C3} cubic}, {\bf \color{C4}
      quartic})}. All models are trained on CIFAR-10 with the same
    initialization + optimization setup, and we plot the
    test logits on the trained models in the first 20 epochs. Each
    point is a 2D PCA embedding of the test logits of the corresponding
    model. Observe that Taylorized training becomes an increasingly better
    approximation of full NN training as we increase the expansion
    order $k$.}
  \label{figure:cnnthick-trajectory}
\end{figure}

==> Sections/plans.tex <==
\section*{TODOs}
\begin{itemize}
% \item Writing (initial pass): intro, related work, conclusion.
\item Resolve the author notes and take a writing pass over the entire
  paper.
\item Cosmetic edits: make plots better, shorten long phrases, % capitalize Taylorized training 
  (e.g. ``theory of linearized training'' to ``linearization
  theory''?), change \{WRNSMALL, WRNWIDE\} to something else.
\item Write proofs for the theoretical result.
\item (Potentially) add more experiments to the appendix.
% \item Motivating questions:
%   \begin{enumerate}[(1)]
%   \item NTK theory are about infinite (or sufficiently high)
%     width. Are they accurate at finite width?
%   \item NTK theory are about initialization; how about at an arbitrary
%     set of parameters?
%   \item What is a superset of \{linearized models\} that approximate
%     neural net training trajectories, yet amenable to theoretical
%     analysis?
%   \end{enumerate}
% \item Our approach: we empirically investigate \emph{Taylorized 
%     training}, i.e. training the first-order 
%   Taylor expansion of a neural network at a certain point.
% \item Result 1: Taylorized models approximate NN training with
%   standard parametrization increasingly better. 
%   \begin{enumerate}[(1)]
%   \item We train neural net and their Taylorized models from the same
%     initialization using same optimziation setups and same SGD
%     randomness. 
%   \item We use the function space distance, i.e. L2 distance between
%     logits on the test dataset, to compare models. We define the
%     \emph{slope} as BLAH. Note that slope = 1 means approximating
%     neural net with the Taylorized model is as bad as approximating
%     with the initialization.
%   \item On both \{CNN, ResNet\}, the slope with all Taylorized models
%     is less than one, and the approximation is better with
%     higher Taylor order.
%   \item Under same optimization setups, the final test performance of
%     Taylorized models is also 
%     monotonely increasing with the order.~\yub{Can we hope to get say
%       within 1\%-2\% test performance using higher-order models?}
%   \item The approximation gets better when we ``branch off'' later in
%     the training.
%   \end{enumerate}
% \item Result 2: We obtain high-performance finite-width Taylorized
%   models.
%   \begin{enumerate}[(1)]
%   \item Maybe with the help of more powerful optimizers,
%     e.g. Adagrad.
%   \item Maybe this alone does not make much sense? Closing the gap is
%     more interesting?
%   \end{enumerate}
% \item Experiments TODO
%   \begin{enumerate}[(1)]
%   \item DONE. Implement function space distance.
%   \item DONE. Quadratic, cubic, and quartic training. 
% % \item \yub{Important:} CIFAR-2 with exact finite-width NTK (compute
% %   in kernel space) and compare with neural net. Maybe ResNet-50 too
% %   strong for that?
% %   \item MetaInit with cross entropy loss on random data.
% %     \begin{enumerate}[(i)]
% %     \item On ResNet50, the meta objective can be optimized from the
% %       inital value of 2.3 to about 0.97. However, the convergence of
% %       SGD / the approximation accuracy of NTK did not get better after
% %       MetaInit.
% %     \item \yub{Try MetaInit on actual training data.}
% %     \end{enumerate}
%   \item WIP. \yub{This is important.}
%     Try out the NTK parametrization (in comparison with the
%     standard NN parametrization.)
%   \item WIP. Try at least one difference architecture, maybe vanilla CNN.
%   \item Use dropout can improve coupling with quadratic models (maybe
%     more than linear models?) This originiated from the randomization
%     idea in~\citep{bai2020beyond}, and can be a pretty cool
%     demonstration that quadratic models plays a meaningful role in
%     practice.
%   \item Try with MSE loss.
%   \end{enumerate}
% \item Theoretical results:
%   \begin{enumerate}[(1)]
%     \item We extend the results of lazy training
%       in~\citep{chizat2019lazy} to Taylorized training.
%   \end{enumerate}
% \item Important papers to compare with and build on:
%   \begin{enumerate}[(1)]
%   \item \citep{chizat2019lazy}: A theory paper on ``lazy training'',
%     i.e. linearized training. Experimented with finite-width
%     linearized network through the ``scaling trick'' (which is the
%     main point of the paper.)
%   \item \citep{park2019effect}: Extensive experiments of network width
%     vs. performance. Can borrow their experimental setups, esp. the
%     balance between what to tune and what to be held fixed.
%   \end{enumerate}
% \item Have a fancier title.
\end{itemize}
